Tahakom LLM Guidelines and Recipes: From Pre-training Data to an Arabic LLM

Large Language Models (LLMs) have significantly advanced the field of natural language processing, enhancing capabilities in both language understanding and generation across diverse domains. However, developing LLMs for Arabic presents unique challenges. This paper explores these challenges by focusing on critical aspects such as data curation, tokenizer design, and evaluation. We detail our approach to the collection and filtration of Arabic pre-training datasets, assess the impact of various tokenizer designs on model performance, and examine the limitations of existing Arabic evaluation frameworks, for which we propose a systematic corrective methodology. To promote transparency and facilitate collaborative development, we share our data and methodologies, contributing to the advancement of language modeling, particularly for the Arabic language.

==> sections/conclusion.tex <==
\section{Conclusion}

This work presents a comprehensive roadmap for developing high-performance Arabic LLMs, addressing key challenges across data curation, tokenization, and evaluation. We contribute a fully filtered Arabic pretraining dataset, validated through ablation studies and supported by open-source tools. Our tokenizer experiments reveal the importance of vocabulary size, data alignment, and method selection in optimizing Arabic model performance. Finally, we enhance the evaluation landscape by improving the benchmark Arabic dataset ARB-MMLU, proposing culturally grounded datasets, and launching a leaderboard for robust Arabic and multilingual model assessment. Together, these contributions establish a robust foundation for the continued development and assessment of Arabic LLMs. We will work on releasing all data and code upon acceptance, aiming to accelerate progress in Arabic NLP and promote more inclusive and equitable language model research across underrepresented languages.

==> sections/related_work.tex <==
\section{Related Work}






